Drift Estimation with Graphical Models

This paper deals with the issue of concept drift in supervised machine learn-ing. We make use of graphical models to elicit the visible structure of the dataand we infer from there changes in the hidden context. Differently from previous concept-drift detection methods, this application does not depend on the supervised machine learning model in use for a specific target variable, but it tries to assess the concept drift as independent characteristic of the evolution of a dataset. Specifically, we investigate how a graphical model evolves by looking at the creation of new links and the disappearing of existing ones in different time periods. The paper suggests a method that highlights the changes and eventually produce a metric to evaluate the stability over time. The paper evaluate the method with real world data on the Australian Electric market.

==> figure0.tex <==
\centering
\begin{equation*}  \label{eu_eqn}
\Tree[.AM_{i,j;t=1}=\{0,1\} 
[.{AM_{i,j;t=2}=\{0\}} {AM_{i,j;t=3}=\{0\}} {AM_{i,j;t=3}=\{1\}} ] 
[.{AM_{i,j;t=2}=\{1\}} {AM_{i,j;t=3}=\{0\}} {AM_{i,j;t=3}=\{1\}} ]  ]
    \end{equation*}

==> figure1.tex <==


\centering
\begin{equation*}  \label{eu_eqn}
\Tree[.\textit{w}_{i,j;t=1}=\{0,1\} 
[.{\textit{w}_{i,j;t=2}=\{0,1\}} {\textit{w}_{i,j;t=3}=\{0,1\}} {\textit{w}_{i,j;t=3}=\{2,3\}} ] 
[.{\textit{w}_{i,j;t=2}=\{2,3\}} {\textit{w}_{i,j;t=3}=\{4,5\}} {\textit{w}_{i,j;t=3}=\{6,7\}} ]  ]
    \end{equation*}





==> materialnotused.tex <==
%%%%spiega perchè serve qullo che segue sulla exchangeabiliy.
%%% il fatto che sono weakly decreasing over time ci serve o è semplicemnte una proprietà interessante?

%%da qui ancora da sisteamre fino al prossimo subsection

In particular we observe that  the sequence of  $Y_k$ is exchangeable respect to the time, because we have build $Y_t$ start from $w_{i,j;t}$:
\begin{equation*}
    \centering
    P(Y_1,...,Y_n)=P(Y_{\sigma(1)},...,Y_{\sigma(n)})
\end{equation*}
for all \begin{math}
n \geq 1
\end{math} and all permutations \begin{math}
\sigma 
\end{math} of \begin{math}
(1,...,n)
\end{math}. In other words, the order of appearance of the observation does not matter in terms of their joint distribution. The structure of the \textit{transition matrix process} will be depend by the spanning forest at time \begin{math}
t=1
\end{math}, and for each year we have a partition of \begin{math}
N
\end{math} given by \begin{math}
\mu_t=\sum_{i=1}^N Y_{i,t}
\end{math} with \begin{math}
t=2,...,T
\end{math}. 





We  observe that the sequence \begin{math}
\{\mu_1,...,\mu_T\}
\end{math} is weakly decreasing over time: 
\begin{equation}
    \mu_{2} \geqslant \mu_{3} \geqslant ... \geqslant \mu_{T} \
\end{equation}
Consequently, this means that the stability of the starting Graph converge to zero in the long period:
\begin{equation}
    \centering
    \mu_t \simeq 0 , \quad  t \rightarrow +\infty
\end{equation}In other words, the random variables in the dataset by changing the relationships between them over time, the joint probability of the dataset \begin{math}
\textbf{X}_t
\end{math} change during the time. It is simple to note that the stability at time 
$t=k$ is equal to time $t=k-1$ when the \textit{Graph} at time $t=k$ is equal at \textit{Graph} at time $t=1$ or when the \textit{Graph} at time   is equal at \textit{Graph} at time $t=k-1$.
The speed of the convergence at \begin{math}
0
\end{math} of the stability, will depend by the number of vertices \begin{math}
V
\end{math} present in the spanning tree.



Specifically, consider tree variables: $Y_i$ as it is defined in Eq. \ref{eq:y}, which capture the stability of a connection

%%%non ho capito cos'è T di i.
$T_i$ which corresponds to the time of transitions between thee first spanning tree until the last spanning tree,  finally 
$W_i$ that maps all possible scenario, whith $i=1,...,n$ where $n= N \times( T-1)$, that is the number of connections per period times the number of transitions.



As a test bed for this theoretical approach, we apply the stability index in a controlled setting of a simulated dataset. We randomly generated 50000 observations from a system of 7 variables over 8 periods and the corresponding 8 graphs. We impose the same relation among variables in $t=1$ and $t=8$ and for $t=4$ and $t=5$ and we investigate the stability over time with respect with $t=1$. Thus, we should observe a declining stability over time with the exception of the 5th and 8th transitions. Equation from \ref{eq:t1} to \ref{eq:t7} in \ref{append} detail the data generation process and Fig.\ref{fig: simulation} portraits the graphs of its empirical realization. 
\begin{figure}[!htbp]
\centering
\begin{tabular}{cc}
% Requires 
\textbf{Spanning Tree $t=1$} & \textbf{Spanning Tree $t=2$}\\
\includegraphics[width=70mm]{images/1.png} &
\includegraphics[width=70mm]{images/2.png}\\
\textbf{Spanning Tree $t=3$} & \textbf{Spanning Tree $t=4$}\\
\includegraphics[width=70mm]{images/3.png}&
\includegraphics[width=70mm]{images/4.png}\\
\textbf{Spanning Tree $t=5$} & \textbf{Spanning Tree $t=6$}\\
\includegraphics[width=70mm]{images/5.png} &
\includegraphics[width=70mm]{images/6.png}\\
\textbf{Spanning Tree $t=7$} & \textbf{Spanning Tree $t=8$}\\
\includegraphics[width=70mm]{images/7.png}&
\includegraphics[width=70mm]{images/8.png}\\
\end{tabular}
\caption{Graph over the time}
 \label{fig: simulation}
\end{figure}
 The Figure \ref{logit} shows the result of the stability for the graphs in Figure \ref{fig: simulation}. On the x-axis, the grpah displays the transition of years (\textit{ty}), in particular we have the comparison do years by years of the \textit{transition matrix}. For instance at when the \begin{math}
ty=1
\end{math} we have the comparison between the graph at \begin{math}
t=1
\end{math} and \begin{math}
t=2
\end{math}. When \begin{math}
ty=4
\end{math} we can see the evolution of the stability between the graphs from \begin{math}
t=1
\end{math} until \begin{math}
t=5
\end{math} and so on.

Figure \ref{logit} shows as the stability decrease from \begin{math}
ty= 1
\end{math} to \begin{math}
ty=3
\end{math}, this means that the relationship between the variables  changes in an evident way. But on the other hand, in period between \begin{math}
ty=3
\end{math} to \begin{math}
ty=5
\end{math} we can see as the \textit{stability} remains flat, this indicates that the relationships between the variables inside the dataset do not change much, and in some cases are the same. Finally, we see how \textit{stability} descends and goes up again. The descend effect is due to the difference in the spanning tree at \begin{math}
 t=7
\end{math} with the previous ones, while the increased effect is due to the fact, the spanning tree at \begin{math}
 t =8
\end{math} is the same as at \begin{math}
t=1
\end{math}.
\begin{figure}
\centering
\textbf{Stability of the graphs over time}\par\medskip
\includegraphics[scale=0.60]{images/Rplot.png}
\caption{Evolution of Stability}
\label{logit}
\end{figure}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table}[!htbp]
\small
\textbf{Regression Summary}\par\medskip
\begin{tabular}{@{}|l|l|@{}}
\toprule
\textbf{Coefficients}    & \textbf{Estimation} \\ \midrule
\textbf{$\beta_0$}       & \textbf{7.66}       \\ \midrule
\textbf{$\beta_{2^T-1}$} & \textbf{19.75}      \\ \midrule
\textbf{$\beta_{Time}$}  & \textbf{-0.30}      \\ \bottomrule
\end{tabular}
\caption{Coefficients of logistic regression }
\label{tab2}
\end{table}

Figure \ref{edgesE} shows the result of the equation \ref{16}, in particular we can see the distribution of the posterior and the evolution of the edges over the time. We can see for each years $\mathcal{V}$ points. Furthermore, Figure \ref{edgesE} shows also as the edges between the variables change over time. Indeed, the ordinate indicates the variables \begin{math}
w_{i,j}
\end{math}, that maps all possible scenario of the connections. 
For instance, if we consider a red point that is close to a yellow point, means that in previous years there was the same behavior between two variables that now it changed. The stability is the connection or not connection will be depend be the value of \textit{w}. In this study, we see that the probability of stability is higher in the first part of the analysis than the second part.
\begin{figure}[!htbp]
\label{edgesE}
\centering
\textbf{Posterior Probability Stability}
\caption{Evolution of the edges}
\includegraphics[scale=0.55]{images/Rplot01.png}
\end{figure}
Figure \ref{PosSta} shows \begin{math} 10000\end{math} samples values of \begin{math}
\beta_0 
\end{math} and \begin{math}
\beta_t
\end{math} from its posterior using a discrete grid approximation to the posterior equation \ref{18}. Finally, Figure \ref{Validation} shows as the model predicts well the evolution of the stability. We have compared the observed data to the posterior predictive. As we can see from Figure \ref{Validation}, the real value (red dot) are inside the credit interval (blue lines).

\begin{figure}[!htbp]
\centering
\textbf{Sampling from posterior}
\caption{Posterior of the Stability}
\includegraphics[scale=0.55]{images/SamplingPosterior.jpg}
\label{PosSta}
\end{figure}






% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}



\begin{table}[!htbp]
\label{tab3}
\caption{Approximation of the drift through the mean \textit{Stability} for each period }
\begin{tabular}{|c|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Percent \\ of Stability\end{tabular}}} & \multicolumn{6}{c|}{\textbf{Evolution of the Drift}}                                                                                                                                                                                                                                                                                                                                               \\ \cline{2-7} 
                                                                                          & {\begin{tabular}[c]{@{}l@{}}$t=2$\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}$t=8$\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}$t=12$\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}$t=14$\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}$t=19$\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}$t=41$\end{tabular}} \\ \hline
\textbf{$ \frac{\sum_{i=1}^N Y_{i,t}}{N}$}                                                & \textbf{$1.0$}                                                  & \textbf{$0.8$}                                                  & \textbf{$0.6$}                                                & \textbf{$0.5$}                                                    & \textbf{$0.2$}                                                   & \textbf{$0.1$}                                                    \\ \hline
\end{tabular}
\end{table}





\section{Validation of the model}
In this section, we present the empirical drift compute in terms of Mean Square Error. We have used the most popular regression tools. In details, we find for each method the best model for the first period and we fit, every single model, for the rest of the periods. The regression tools used are the \textit{random forest regression}, the \textit{ordinary least squares}, The \textit{support vector machine} and the\textit{ lasso method} \citep{friedman2001elements}.

\begin{figure}[!htbp]
\centering
\begin{tabular}{cc}
% Requires 
\textbf{Evolution of Random Forest MSE} & \textbf{Evolution of OLS MSE}\\
\includegraphics[width=75mm]{images/RF.png} &
\includegraphics[width=75mm]{images/OLS.png}\\
\textbf{Evolution of SVM MSE} & \textbf{Evolution of LASSO MSE}\\
\includegraphics[width=75mm]{images/SVM.png}&
\includegraphics[width=75mm]{images/LAsso.png}\\
\end{tabular}
\caption{Empirical drift}
 \label{comparison}
\end{figure}
Figure \ref{comparison} shows as the \textit{MSE} changes over the time for each period. It is important to note that, when the \textit{stability} is flat,the\textit{ MSE} decreases otherwise when the \textit{stability} decreases the \textit{MSE} increases. 

\begin{appendices}
\label{append}
 The dataset is composed by $50000$ observations and by 7 variables (all of them continuous) that we have call them $X_i,Y_i,Z_i,W_i,S_i,H_i$ and $T_i$. We have build the dataset to control relationship between the variables and to test if the there is not change in datasets form one period to other, the \textit{stability} will still be the same. For the $t=1$ the dataset is composed in the following way:
\begin{equation} 
\label{eq:t1}
t=1 \:and\: t=8
\begin{cases}
 X_i& \sim  N(\mu=5; \sigma=100) \\ 
Y_i& \sim N(\mu=0; \sigma=3) +0.8\times X_i\\
Z_i& \sim \text{Unif} (a=0; b=1) +0.2\times Y_i\\
W_i& \sim \text{Unif} (a=0; b=1) +0.5\times X_i\\
S_i& \sim \text{Unif} (a=1; b=4) +0.89\times Z_i\\
H_i& \sim \text{Unif} (a=1; b=5000) +Z_i\\
T_i& \sim \text{Unif} (a=0; b=1) +0.5\times H_i\\  
\end{cases}
\end{equation}

\begin{equation} 
t=2
\begin{cases}
X_i& \sim  N(\mu=5; \sigma=100) \\ 
Y_i& \sim N(\mu=0; \sigma=3) +0.8\times X_i\\
Z_i& \sim \text{Unif} (a=1; b=5000) +0.2\times Y_i\\
W_i& \sim \text{Unif} (a=0; b=1) +0.5\times X_i\\
S_i& \sim \text{Unif} (a=1; b=4) +0.89\times Z_i\\
H_i& \sim \text{Unif} (a=1; b=5000) +0.5\times Z_i\\
T_i& \sim \text{Unif} (a=0; b=1) +0.5\times W_i\\
\end{cases}
\end{equation}

\begin{equation} 
t=3
\begin{cases}
X_i& \sim  N(\mu=5; \sigma=100) \\ 
Y_i& \sim N(\mu=0; \sigma=3) +0.8\times X_i\\
Z_i& \sim \text{Unif} (a=1; b=5000) +0.2\times Y_i\\
W_i& \sim \text{Unif} (a=0; b=1) +0.5\times X_i\\
S_i& \sim \text{Unif} (a=1; b=4) +0.89\times Z_i\\
H_i& \sim \text{Unif} (a=1; b=5000) +0.5\times Z_i\\
T_i& \sim \text{Unif} (a=0; b=1) +0.5\times W_i\\
\end{cases}
\end{equation}

\begin{equation}
t=4 \:and \: t=5
\begin{cases}
X_i& \sim  N(\mu=5; \sigma=100) \\ 
Y_i& \sim N(\mu=0; \sigma=3) +0.8\times X_i\\
Z_i& \sim \text{Unif} (a=1; b=5000) +0.2\times Y_i\\
W_i& \sim \text{Unif} (a=0; b=1) +0.5\times X_i\\
S_i& \sim \text{Unif} (a=1; b=4) +0.89\times Z_i\\
H_i& \sim \text{Unif} (a=1; b=5000) +0.5\times Z_i\\
T_i& \sim \text{Unif} (a=0; b=1) +0.5\times W_i+0.89\times W_i\\
\end{cases}
\end{equation}

\begin{equation} 
t=6
\begin{cases}
X_i& \sim  N(\mu=5; \sigma=100) \\ 
Y_i& \sim N(\mu=0; \sigma=3) +0.8\times X_i\\
Z_i& \sim \text{Unif} (a=1; b=5000) +0.2\times Y_i\\
W_i& \sim \text{Unif} (a=0; b=1) +0.5\times X_i\\
S_i& \sim \text{Unif} (a=1; b=4) +0.89\times Y_i\\
H_i& \sim \text{Unif} (a=1; b=5000) +0.5\times Y_i+0.89\times X_i\\
T_i& \sim \text{Unif} (a=0; b=1) +0.89\times W_i\\
\end{cases}
\end{equation}

\begin{equation} 
\label{eq:t7}
t=7
\begin{cases} 
X_i& \sim  N(\mu=5; \sigma=100) \\ 
Y_i& \sim N(\mu=0; \sigma=3) +0.8\times X_i\\
Z_i& \sim \text{Unif} (a=1; b=5000) +0.2\times Y_i\\
W_i& \sim \text{Unif} (a=0; b=1) +0.5\times X_i\\
S_i& \sim \text{Unif} (a=1; b=4) +0.89\times Y_i\\
H_i& \sim \text{Unif} (a=1; b=5000) +0.5\times Y_i+0.89\times W_i\\
T_i& \sim \text{Unif} (a=0; b=1) +0.5\times Y_i+0.89\times X_i\\
\end{cases}
\end{equation}


\end{appendices}


We model \begin{math}
Y_{1;k}=y_{1;k},...,Y_{N;k}=y_{N;k}
\end{math} using the Bayesian \textit{Beta-Bernulli Model}: 
\begin{align*}
y_{1;k},...,y_{N;k} | \theta_k \thicksim \text{Ber}\{\theta_k\}\\
\theta_k \thicksim \text{Beta}(a_k,b_k) \\ k=2,..,t
 \end{align*}
where \begin{math}
\theta_k
\end{math} represents the latent random variable of \textit{stability of the Graph} during the time. At time  \begin{math}
k=2
\end{math} we use [...]\\
We define with \begin{math}
\mu_k
\end{math} as mean of the sampling model, \begin{math}
\mu_k= \frac{\sum_{i=N}y_i}{N}
\end{math}. We  observe that the sequence \begin{math}
\{\mu_1,...,\mu_k\}
\end{math} is weakly decreasing over time: 
\begin{equation}
    \mu_{2} \geqslant \mu_{3} \geqslant ... \geqslant \mu_{t} \
\end{equation}
Consequently, this means that the stability of the starting Graph converge to zero in the long period:
\begin{equation}
    \centering
    \theta_t \simeq 0 , \quad  t \rightarrow +\infty
\end{equation}In other words, the random variables in the dataset by changing the relationships between them over time, the joint probability of the dataset \begin{math}
\textbf{X}_k
\end{math} change during the time. We prove  with an example that stability at time \begin{math}
t=k
\end{math} is equal to time \begin{math}
t=k-1
\end{math} when the \textit{Graph} at time \begin{math}
t=k
\end{math} is equal at \textit{Graph} at time \begin{math}
t=1
\end{math} or when the \textit{Graph} at time \begin{math}
t=k
\end{math}  is equal at \textit{Graph} at time \begin{math}
t=k-1
\end{math}.

